Segmenting Object Affordances: Reproducibility and Sensitivity to Scale

Visual affordance segmentation identifies image regions of an object an agent can interact with. Existing methods re-use and adapt learning-based architectures for semantic segmentation to the affordance segmentation task and evaluate on small-size datasets. However, experimental setups are often not reproducible, thus leading to unfair and inconsistent comparisons. In this work, we benchmark these methods under a reproducible setup on two single objects scenarios, tabletop without occlusions and hand-held containers, to facilitate future comparisons. We include a version of a recent architecture, Mask2Former, re-trained for affordance segmentation and show that this model is the best-performing on most testing sets of both scenarios. Our analysis shows that models are not robust to scale variations when object resolutions differ from those in the training set.

==> tex/training_setup_umd.tex <==
\begin{table}[t!]
    \centering
    % \footnotesize
    \scriptsize
    \setlength\tabcolsep{1pt}
    \caption{Our training setup of affordance segmentation methods for the UMD dataset~\cite{myers2015affordance}. }
    \begin{tabular}{r r r c c c c c l l c r c}
    \toprule
    \textbf{Model} & \textbf{Back} & \textbf{Resolution} & \multicolumn{4}{c}{\textbf{Augmentation}} & \textbf{Resize} & \multicolumn{5}{c}{\textbf{Parameters}} \\
    \cmidrule(lr){4-7}\cmidrule(lr){9-13}
    & & & FL & SCA & ROT & CJ & (Tr/Ts) & Optim. & LR & Mom. & WD & Batch \\
    \midrule
    CNN~\cite{nguyen2016detecting} & VG16 & $640 \times 480$ & $\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & cc/NC & Adam & $10^{-3}$ & - & 0 & 4 \\ 
    DRNAtt~\cite{gu2021visual} & DR22 & $640 \times 480$ & $\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & cc/NC & Adam & $10^{-3}$ & - & 0 & 4 \\
    AffNet~\cite{do2018affordancenet} & RN50 & $640 \times 480$ & $\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & cc/NC & MGD & $10^{-3}$ & - & $10^{-3}$ & 2 \\ % .001 | 
    % GSE~\cite{zhang2022multi} \\ % & $400 \times 400$ & $\bullet$ & $\bullet$ & $\circ$ & $\circ$ & c/- & - & $10^{-3}$ & .9 & $10^{-4}$ & - \\ % $[0.5 - 2]$
    M2Former~\cite{cheng2022masked} & RN50 & $640 \times 480$ & $\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & cc/NC & AdamW & $10^{-4}$ & - & 0 & 4 \\
    LANet & RN50 & $640 \times 480$ & $\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & cc/NC & AdamW & $10^{-4}$ & - & 0 & 4\\ 
    %RANet~\cite{zhao2020object} & $224 \times 224$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & cc/- & Adam & $10^{-4}$ & - & - & - \\
    %BPN~\cite{yin2022object} & $1000 \times 600$  & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & - & - & $10^{-3}$ & .9 & $10^{-4}$ & 4\\ %  $[- 30, 30]$, $[0.5, 1.25]$, $[- 10, 10]$ 
    \bottomrule
    \addlinespace[\belowrulesep]
    \multicolumn{13}{l}{\parbox{0.95\linewidth}{\scriptsize{KEYS -- FL:~flipping, SCA:~scaling, ROT:~rotating, CJ:~color jittering, (Tr/Ts): resize procedure in training and testing, Optim.:~training optimiser,  LR:~initial learning rate, Mom.:~ momentum, WD:~weight decay, Batch: batch size, AffNet:~AffordanceNet, cc:~centre-crop, c:~crop, sw:~sliding window, MGD:~Mini-batch gradient descent, NC:~no image cropping, -:~not specified,   $\bullet$:~considered, $\circ$:~not considered.}}}\\
    \end{tabular}
    \label{tab:umdtrainingsetup}
\end{table}

